Auditing the Imputation Effect on Fairness of Predictive Analytics in Higher Education

Colleges and universities use predictive analytics in a variety of ways to increase student success rates. Despite the potential for predictive analytics, two major barriers exist to their adoption in higher education: (a) the lack of democratization in deployment, and (b) the potential to exacerbate inequalities. Education researchers and policymakers encounter numerous challenges in deploying predictive modeling in practice. These challenges present in different steps of modeling including data preparation, model development, and evaluation. Nevertheless, each of these steps can introduce additional bias to the system if not appropriately performed. Most large-scale and nationally representative education data sets suffer from a significant number of incomplete responses from the research participants. While many education-related studies addressed the challenges of missing data, little is known about the impact of handling missing values on the fairness of predictive outcomes in practice. In this paper, we set out to first assess the disparities in predictive modeling outcomes for college-student success, then investigate the impact of imputation techniques on the model performance and fairness using a commonly used set of metrics. We conduct a prospective evaluation to provide a less biased estimation of future performance and fairness than an evaluation of historical data. Our comprehensive analysis of a real large-scale education dataset reveals key insights on modeling disparities and how imputation techniques impact the fairness of the student-success predictive outcome under different testing scenarios. Our results indicate that imputation introduces bias if the testing set follows the historical distribution. However, if the injustice in society is addressed and consequently the upcoming batch of observations is equalized, the model would be less biased.

==> dataset.tex <==
\section{Dataset}
We select a subset of influential attributes including students' demographic information, socio-economic status, family and environmental factors, grades and achievements, and extra activities. 
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[!htbp]
  \centering
    \begin{adjustbox}{width=1\columnwidth}
   \begin{tabular}{|l|c|l|c|}
    \toprule
    \textbf{Variables } & \textbf{\% Missing} & \textbf{Variables } & \textbf{\% Missing} \\
    \midrule
    S-T relationship & 38.97 & Number of school activities & 1.07 \\
    \midrule
    F3-loan-owed & 31.23 & Std Math/Reading & 0.03 \\
    \midrule
    \%white teacher & 27.05 & English & 0.03 \\
    \midrule
    \%Black teacher & 23.76 & High school attendance & 0.02 \\
    \midrule
    \%Hispanic teacher & 21.94 & Family Composition & 0 \\
    \midrule
    F3\_GPA(first year) & 16.54 & Race\_Hispanic, race specified & 0 \\
    \midrule
    TV/video(h/day) & 15.68 & F3\_Separated no partner & 0 \\
    \midrule
    F3\_GPA(first attended) & 15.09 & F3\_Never Married w partner & 0 \\
    \midrule
    Work(h/week) & 14.24 & F3\_Never Married no partner & 0 \\
    \midrule
    F2\_College entrance & 12.74 & F3\_Married & 0 \\
    \midrule
    credits (first year) & 11.4  & F3\_Divorced/Widowed w partner & 0 \\
    \midrule
    F3\_GPA(all) & 10.58 & F3\_Divorced/Widowed no partner & 0 \\
    \midrule
    F1\_TV/video(h/day) & 10.52 & Race\_White & 0 \\
    \midrule
    Credits (total) & 10.2  & Race\_More than one race & 0 \\
    \midrule
    Generation & 9.76  & Race\_Hispanic, no race specified & 0 \\
    \midrule
    F3\_Credits\_ math  & 9.22  & School Urbanicity & 0 \\
    \midrule
    F3\_Credits\_Science & 9.21  & Race\_Black or African Amer & 0 \\
    \midrule
    F3\_Highest level of education & 7.58  & Race\_Asian, Hawaii/Pac. Isl & 0 \\
    \midrule
    F3\_Employment & 7.58  & Race\_Amer. Indian/Alaska & 0 \\
    \midrule
    F1\_Std Math & 7.54  & Gender\_Male & 0 \\
    \midrule
    F1\_frequency of computer use & 6.64  & Gender\_Female & 0 \\
    \midrule
    F1\_units in math & 6.15  & Parents education & 0 \\
    \midrule
    Athletic level & 5.59  & Income & 0 \\
    \midrule
    F1\_Work(h/week) & 4.4   & F1\_Drop out & 0 \\
    \midrule
    Homework(h/week) & 2.37  & F3\_Separated w partner & 0 \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
  \label{tab:Missings}%
\end{table}%




==> tradeoff.tex <==
\section{Fairness-Accuracy Trade-off}

Imagine a situation that one of the protected attributes, e.g. race, is highly correlated with the target variable (e.g., highest degree attained). As a result, a biased yet accurate model predicts a low target value (e.g., lower degree) for individuals in specific racial groups. 
In this case, enforcing the model to satisfy a fairness constraint during the training, prevents it to relate race with the predicted highest level of education. 
This procedure might decrease the model accuracy but achieves higher fairness for protected groups. Indeed, the ideal goal of fairness in ML may not be possible in all problems as some existing works have pointed out that an inherent trade-off exists between fairness and accuracy \cite{fair-trade-off,fair-trade-off2,fair-trade-off3}. In other words, prediction accuracy needs to be sacrificed to some extent in order to lower prediction bias \cite{fair-trade-off3,fair-trade-off4,fair-tradeoff-main}. 
To balance the fairness and accuracy trade-off, some recent works considered a Pareto frontier construction (multiple objective optimization techniques) \cite{fair-trade-off-pareto1,fair-trade-off-pareto2} based on fairness and accuracy or proposed. 




In this proposal, we aim to consider a classification ( categorical response: e.g. Attainment)
problem to predict student success. While some ML models can only be used for either regression or classification problems, some others can be applied to both problems after necessary modifications. Decision Tree \cite{DT-corr-perform,DT-admission,DT-impfactor,SVM-DT-RF-NN}, Random Forest \cite{RF-Progression,RF-risk,SVM-DT-RF-NN}, Neural Network \cite{SVM-NN,SVM-DT-NN,SVM-DT-RF-NN,NN}, and SVM \cite{SVM-DT-NN,SVM-DT-RF-NN,SVM-KNN,SVM-NN} are among the well-known models in higher education that can be applied for both regression and classification problems. Moreover, some models are interpretable (e.g Decision Tree~\cite{DT-admission}) while others require extra effort for interpretation (e.g Nural Netwrok~\cite{explainableAI}). The ability to explain the rationale behind each prediction outcome is a necessity in human-related fields such as education. As a result, we prefer interpretable models due to their explainability for higher education researchers. However, we investigate the non-interpretable ones as well and provide insights on how to extract useful information from them using explainable AI techniques \cite{explainableAI,explainableAI2}.  

